Solving Inverse Problems in Medical Imaging with Score-Based Generative Models

Reconstructing medical images from partial measurements is an important inverse problem in Computed Tomography (CT) and Magnetic Resonance Imaging (MRI). Existing solutions based on machine learning typically train a model to directly map measurements to medical images, leveraging a training dataset of paired images and measurements. These measurements are typically synthesized from images using a fixed physical model of the measurement process, which hinders the generalization capability of models to unknown measurement processes. To address this issue, we propose a fully unsupervised technique for inverse problem solving, leveraging the recently introduced score-based generative models. Specifically, we first train a score-based generative model on medical images to capture their prior distribution. Given measurements and a physical model of the measurement process at test time, we introduce a sampling method to reconstruct an image consistent with both the prior and the observed measurements. Our method does not assume a fixed measurement process during training, and can thus be flexibly adapted to different measurement processes at test time. Empirically, we observe comparable or better performance to supervised learning techniques in several medical imaging tasks in CT and MRI, while demonstrating significantly better generalization to unknown measurement processes.

==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/abs.tex <==
\begin{abstract}



Reconstructing medical images from partial measurements is an important inverse problem in Computed Tomography (CT) and Magnetic Resonance Imaging (MRI). Existing solutions based on machine learning typically train a model to directly map measurements to medical images, leveraging a training dataset of paired images and measurements. These measurements are typically synthesized from images using a fixed physical model of the measurement process, which hinders the generalization capability of models to unknown measurement processes. To address this issue, we propose a fully unsupervised technique for inverse problem solving, leveraging the recently introduced score-based generative models. Specifically, we first train a score-based generative model on medical images to capture their prior distribution. Given measurements and a physical model of the measurement process at test time, we introduce a sampling method to reconstruct an image consistent with both the prior and the observed measurements. Our method does not assume a fixed measurement process during training, and can thus be flexibly adapted to different measurement processes at test time. Empirically, we observe comparable or better performance to supervised learning techniques in several medical imaging tasks in CT and MRI, while demonstrating significantly better generalization to unknown measurement processes.
\end{abstract}

==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/background.tex <==
\section{Background}\label{sec:background}

\subsection{Linear inverse problems}
An inverse problem seeks to recover an unknown signal from a set of observed measurements. Specifically, suppose $\rvx \in \mbb{R}^n$ is an unknown signal, and $\rvy \in \mbb{R}^m = \mA \rvx + \bm{\epsilon}$ is a noisy observation given by $m$ linear measurements, where the measurement acquisition process is represented by a linear operator $\mA \in \mbb{R}^{m\times n}$, and $\bm{\epsilon} \in \mbb{R}^n$ represents a noise vector. Solving a linear inverse problem amounts to recovering the signal $\rvx$ from its measurement $\rvy$. Without further assumptions, the problem is ill-defined when $m < n$, so we additionally assume that $\rvx$ is sampled from a prior distribution $p(\rvx)$. In this probabilistic formulation, the measurement and signal are connected through a measurement distribution $p(\rvy \mid \rvx) = q_{\bm{\epsilon}}(\rvy - \mA \rvx)$, where $q_{\bm{\epsilon}}$ denotes the noise distribution of $\bm{\epsilon}$. 
Given $p(\rvy \mid \rvx)$ and $p(\rvx)$, we can solve the inverse problem by sampling from the posterior distribution $p(\rvx \mid \rvy)$.


Examples of linear inverse problems in medical imaging include image reconstruction for CT and MRI. In both cases, the signal $\rvx$ is a medical image. The measurement $\rvy$ in CT is a sinogram formed by X-ray projections of the image from various angular directions~\citep{buzug2011computed}, while the measurement $\rvy$ in MRI consists of spatial frequencies in the Fourier space of the image (\aka the k-space in the MRI community)~\citep{vlaardingerbroek2013magnetic}.

\subsection{Score-based generative models}\label{sec:sbgm}
When solving inverse problems in medical imaging, we are given an observation $\rvy$, the measurement distribution $p(\rvy \mid \rvx)$ and aim to sample from the posterior distribution $p(\rvx \mid \rvy)$. The prior distribution $p(\rvx)$ is typically unknown, but we can train generative models on a dataset $\{\rvx^{(1)}, \rvx^{(2)}, \cdots, \rvx^{(N)}\} \sim p(\rvx)$ to estimate this prior distribution. Given an estimate of $p(\rvx)$ and the measurement distribution $p(\rvy \mid \rvx)$, the posterior distribution $p(\rvx \mid \rvy)$ can be determined through Bayes' rule.

We propose to estimate the prior distribution of medical images using the recently introduced score-based generative models~\citep{song2019generative,ho2020denoising,song2021scorebased}, whose iterative sampling procedure makes it especially easy for controllable generation conditioned on an observation $\rvy$. Specifically, we adopt the formulation of score-based generative models in \citet{song2021scorebased}, where we leverage a Markovian diffusion process to progressively perturb data to noise, and then smoothly convert noise to samples of the data distribution by estimating and simulating its time reversal. %
We provide an illustration of this generative modeling framework in \cref{fig:sde}.

\begin{SCfigure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/sde_schematic.jpg}
    \caption{We can smoothly perturb images to noise by following the trajectory of an SDE. By estimating the score function $\nabla_\rvx \log p_t(\rvx)$ with neural networks (called score models), it is possible to approximate the reverse SDE and then solve it to generate image samples from noise.}
    \label{fig:sde}
\end{SCfigure}

\textbf{Perturbation process}~
Suppose the dataset is sampled from an unknown data distribution $p(\rvx)$. We perturb datapoints with a stochastic process over a time horizon $[0, 1]$, governed by a linear stochastic differential equation (SDE) of the following form
\begin{align}
        \ud \rvx_t = f(t)\rvx_t \ud t + g(t) \ud \rvw_t,  \qquad t \in [0, 1],\label{eq:sde}
\end{align}
where $f: [0,1] \to \mbb{R} $, $g: [0,1] \to \mbb{R}$, $\{\rvw_t \in \mbb{R}^n\}_{t\in[0,1]} $ denotes a standard Wiener process (\aka, Brownian motion), and $\{\rvx_t \in \mbb{R}^n \}_{t \in [0, 1]}$ symbolizes the trajectory of random variables in the stochastic process. We further denote the marginal probability distribution of $\rvx_t$ as $p_t(\rvx)$, and the transition distribution from $\rvx_0$ to $\rvx_t$ as $p_{0t}(\rvx_t \mid \rvx_0)$. By definition, we clearly have $p_0(\rvx) \equiv p(\rvx)$. Moreover, the functions $f(t)$ and $g(t)$ are specifically chosen such that for any initial distribution $p_0(\rvx)$, the distribution at the end of the perturbation process, $p_1(\rvx)$, is close to a pre-defined noise distribution $\pi(\rvx)$. In addition, the transition density $p_{0t}(\rvx_t \mid \rvx_0)$ is always a conditional linear Gaussian distribution, taking the form $p_{0t}(\rvx_t \mid \rvx_0) = \mcal{N}(\rvx_t \mid \alpha(t) \rvx_0, \beta^2(t)\mI)$ where $\alpha: [0,1] \to \mbb{R}$ and $\beta: [0,1] \to \mbb{R}$ can be derived analytically from $f(t)$ and $g(t)$~\citep{sarkka2019applied}. Examples of such SDEs include Variance Exploding (VE), Variance Preserving (VP), and subVP SDEs proposed in~\citet{song2021scorebased}. We found VE SDEs performed the best in our experiments. 



\textbf{Reverse process}~
By reversing the perturbation process in \cref{eq:sde}, we can start from a noise sample $\rvx_1 \sim p_1(\rvx)$ and gradually remove the noise therein to obtain a data sample $\rvx_0 \sim p_0(\rvx) \equiv p(\rvx)$. Crucially, the time reversal of \cref{eq:sde} is given by the following reverse-time SDE~\citep{song2021scorebased}
\begin{align}
    \ud \rvx_t = \left[ f(t)\rvx_t - g(t)^{2} \nabla_{\rvx_t} \log p_{t}(\rvx_t) \right] \ud t + g(t) \ud \bar{\rvw}_t,\qquad t\in[0,1], \label{eq:reverse_sde}
\end{align}
where $ \{\bar{\rvw}_t\}_{t\in[0, 1]} $ denotes a standard Wiener process in the reverse-time direction, and $\ud t$ represents an infinitesimal negative time step, since the above SDE must be solved backwards from $t=1$ to $t=0$. The quantity $\nabla_{\rvx_t}\log p_{t}(\rvx_t)$ is known as the \emph{score function} of $p_t(\rvx_t)$. By the definition of time reversal, the trajectory of the reverse stochastic process given by \cref{eq:reverse_sde} is $\{\rvx_t\}_{t\in [0,1]}$, same as the one from the forward SDE in \cref{eq:sde}.

\textbf{Sampling}~
Given an initial sample from $p_1(\rvx)$, as well as scores at each intermediate time step, $\nabla_\rvx \log p_t(\rvx)$, we can simulate the reverse-time SDE in \cref{eq:reverse_sde} to obtain samples from the data distribution $p_0(\rvx) \equiv p(\rvx)$. In practice, the initial sample is approximately drawn from $\pi(\rvx)$ since $\pi(\rvx) \approx p_1(\rvx)$, and the scores are estimated by training a neural network $\vs_\vtheta(\rvx, t)$ (named the \emph{score model}) on a dataset $\{\rvx^{(1)}, \rvx^{(2)}, \cdots, \rvx^{(N)}\} \sim p(\rvx)$ with denoising score matching~\citep{vincent2011connection,song2021scorebased}, \ie, solving the following objective
\begin{align*}
    \vtheta^* = \argmin_\vtheta \frac{1}{N}\sum_{i=1}^N \mbb{E}_{t \sim \mcal{U}[0, 1]}\mbb{E}_{\rvx_t^{(i)} \sim p_{0t}(\rvx_t^{(i)} \mid \rvx^{(i)})}\Big[\norm{\vs_{\vtheta}(\rvx^{(i)}_t, t) - \nabla_{\rvx^{(i)}_t} \log p_{0t}(\rvx_t^{(i)} \mid \rvx^{(i)})}_2^2\Big],
\end{align*}
where $\mcal{U}[0,1]$ denotes a uniform distribution over $[0, 1]$. The theory of denoising score matching ensures that $\vs_{\vtheta^*}(\rvx, t) \approx \nabla_\rvx \log p_t(\rvx)$. After training this score model, we plug it into \cref{eq:reverse_sde} and solve the resulting reverse-time SDE
\begin{align}
    \ud \rvx_t = \left[ f(t)\rvx_t - g(t)^{2} \vs_{\vtheta^*}(\rvx_t, t) \right] \ud t + g(t) \ud \bar{\rvw}_t, \qquad t\in[0,1 ], \label{eq:reverse_sde_model}
\end{align}
for sample generation. One sampling method is to use the Euler-Maruyama discretization for solving \cref{eq:reverse_sde_model}, as given in \cref{alg:sampling}. 
Other sampling methods include annealed Langevin dynamics~\citep[ALD,][]{song2019generative}, probability flow ODE solvers~\citep{song2021scorebased}, and Predictor-Corrector samplers~\citep{song2021scorebased}. %



==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/cmd.tex <==

\usepackage{amsmath,amsfonts,bm,amssymb,mathtools,amsthm}
\usepackage{color,xcolor}

\usepackage{hyperref}       %
\hypersetup{
  colorlinks,
  linkcolor={red!50!black},
  citecolor={blue!50!black},
  urlcolor={blue!80!black}
  }
  \definecolor{orange}{HTML}{ff7f0e}
  \definecolor{blue}{HTML}{1f77b4}
  
\usepackage{url}
\usepackage{xkcdcolors}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{algorithmicx}

\usepackage{microtype}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{latexsym}
\usepackage{sidecap}
\usepackage{caption}
\usepackage{booktabs} %
\usepackage{amsfonts}       %
\usepackage{nicefrac}       %
\usepackage{comment}
\usepackage{enumitem}
\usepackage{wrapfig,tikz}
\usepackage{longtable,fancyhdr}
\usepackage{adjustbox, bigstrut, tabularx, multirow, makecell, diagbox}
\usepackage{float}
\usepackage{stackrel}
\usepackage{color}
\usepackage{colortbl}
\usepackage{theoremref}
\usepackage{cases}
\usepackage{stmaryrd}
\usepackage{mathabx}
\usepackage{dsfont}
\usepackage{arydshln}

\usepackage[capitalise]{cleveref}


\makeatletter
\usepackage{xspace} 
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}

\definecolor{blue1}{RGB}{0,128,255}
\definecolor{blue3}{RGB}{0,0,128}
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand*{\tran}{^{\mkern-1.5mu\mathsf{T}}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\mcal}[1]{\mathcal{#1}}
\newcommand{\mrel}{\mathrel}

\def\eg{\emph{e.g}\onedot}
\def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot}
\def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot}
\def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot}
\def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot}
\def\resp{resp\onedot}
\def\dof{d.o.f\onedot}
\def\aka{a.k.a\onedot}
\def\iid{i.i.d\onedot}
\def\etal{\emph{et al}\onedot}

\definecolor{darkgreen}{rgb}{0,0.6,0}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}

\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vpi{{\bm{\pi}}}
\def\vomega{{\bm{\omega}}}
\def\vlambda{{\bm{\lambda}}}
\def\vphi{{\bm{\phi}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\psde}{p_\vtheta^{\textnormal{SDE}}}
\newcommand{\ptsde}{\tilde{p}_\vtheta^{\textnormal{SDE}}}
\newcommand{\pode}{p_\vtheta^{\textnormal{ODE}}}
\newcommand{\ptode}{\tilde{p}_\vtheta^{\textnormal{ODE}}}
\newcommand{\boundsm}{\mcal{L}^{\text{SM}}_\vtheta}
\newcommand{\bounddsm}{\mcal{L}^{\text{DSM}}_\vtheta}
\newcommand{\jsm}{\mcal{J}_{\textnormal{SM}}}
\newcommand{\jdsm}{\mcal{J}_{\textnormal{DSM}}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\ud}{\mathop{}\!\mathrm{d}}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\let\ab\allowbreak


==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/conclusion.tex <==
\section{Conclusion}
We propose a new method to solve linear inverse problems with score-based generative models. Our method is fully unsupervised, requires no paired data for training, can flexibly adapt to different measurement processes at test time, and only requires minimal modifications to a large number of existing sampling methods of score-based generative models. Empirical results demonstrate that our method can match or outperform existing supervised learning counterparts on image reconstruction for sparse-view CT and undersampled MRI, and has better generalization to new measurement processes, such as using a different number of projections or downsampling ratios in CT/MRI, and tackling both sparse-view CT reconstruction and metal artifact removal with a single model.

\subsubsection*{Author Contributions}
Yang Song designed the project, wrote the paper, and ran all experiments for score-based generative models. Liyue Shen preprocessed data, ran all baseline experiments, and helped write the paper. Lei Xing and Stefano Ermon supervised the project, provided valuable feedback, and helped edit the paper.

\subsubsection*{Acknowledgments}
YS is supported by the Apple PhD Fellowship in AI/ML. LS is supported by the Stanford Bio-X Graduate Student Fellowship. This research was supported by NSF (\#1651565, \#1522054, \#1733686), ONR (N000141912145), AFOSR (FA95501910024), ARO (W911NF-21-1-0125), Sloan Fellowship, and Google TPU Research Cloud. This research was also supported by NIH/NCI (1R01 CA256890 and 1R01 CA227713).

 
 
 



==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/experiments.tex <==

\section{Experiments}

We aim to answer the following questions in this section: (1) Can we directly compete with best-in-class supervised learning techniques for the same measurement process used in their training, even though our approach is fully unsupervised? (2) Can our method generalize better to new measurement processes?  (3) How do we fare against other unsupervised approaches? To study these questions, we experiment on several tasks in medical imaging, including sparse-view CT reconstruction, metal artifact removal (MAR) for CT, and undersampled MRI reconstruction. More experimental details are provided in \cref{app:exp}.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_fista_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_fista_demo.png}
        \caption{FISTA-TV}
    \end{subfigure}
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_cgan_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_cgan_demo.png}
        \caption{cGAN}
    \end{subfigure}
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_neumann_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_neumann_demo.png}
        \caption{Neumann}
    \end{subfigure}
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_sin_prn_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_sin_prn_demo.png}
        \caption{SIN-4c-PRN}
    \end{subfigure}
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_ours_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_ours_demo.png}
        \caption{Ours}
    \end{subfigure}
    \begin{subfigure}[b]{0.161\textwidth}
        \includegraphics[width=\linewidth]{figures/lidc_gt_demo.png}
        \includegraphics[width=\linewidth]{figures/ldct_gt_demo.png}
        \caption{Ground truth}
    \end{subfigure}
    \caption{Examples of sparse-view CT reconstruction results on LIDC $320\times 320$ \emph{(Top row)} and LDCT $512\times 512$ \emph{(Bottom row)}, all with 23 projections. You may zoom in to view more details.}
    \label{fig:ct_demo}
\end{figure}

\textbf{Datasets}~
We consider two datasets for CT experiments. The first is the Lung Image Database Consortium (LIDC) image collection dataset ~\citep{armato2011lidclung, clark2013tcia} where we slice the original 3D CT volumes to obtain 130304 2D images of resolution $320\times 320$ for training. The second is the Low Dose CT (LDCT) Image and Projection dataset~\citep{moen2021ldct} that contains CT scans of multiple anatomic sites, including head, chest, and abdomen, from which we generate 47006 2D image slices of resolution $512\times 512$ for training. 
We simulate CT measurements (sinograms) with a parallel-beam geometry using projection angles equally distributed across 180 degrees. For MAR experiments, we follow \cite{yu2020deep} to synthesize metal artifacts.
For undersampled MRI experiments, we use the Brain Tumor Segmentation (BraTS) 2021 dataset~\citep{menze2014brats, bakas2017brats2}, where we slice 3D MRI volumes to get 297270 images of resolution $240 \times 240$ as the training dataset. We simulate MRI measurements with Fast Fourier Transform using a single-coil setup, and follow~\citet{zbontar2018fastMRI,knoll2020fastmri} to undersample the k-space with an equispaced Cartesian mask. The performance is measured on 1000 test images with peak signal-to-noise ratio (PSNR) and structural similarity (SSIM). 

\textbf{Standard techniques in medical imaging}~
We include two standard learning-free techniques as baselines for sparse-view CT reconstruction. The first is filtered back projection on sparse-view sinograms, which is denoted by ``FBP''. The second is an iterative reconstruction method with total variation regularization called FISTA-TV~\citep{beck2009fista}. For MAR experiments, we include another learning-free baseline called linear interpolation~\citep[LI,][]{kalender1987reduction}.

\begin{table}
    \definecolor{h}{gray}{0.9}
    \caption{Results for undersampled MRI reconstruction on BraTS. First two methods are supervised learning techniques trained with $8\times $ acceleration. The others are unsupervised techniques. \label{tab:mri}}
    \centering
    {\setlength{\extrarowheight}{1.5pt}
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{c|cc|cc|cc}
    \Xhline{3\arrayrulewidth}
    \multirow{2}{*}[-1pt]{Method}  & \multicolumn{2}{c|}{24$\times$ Acceleration} & \multicolumn{2}{c|}{8$\times$ Acceleration} & \multicolumn{2}{c}{4$\times$ Acceleration} \\\cline{2-7}
    & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$\\
    \hline
    Cascade DenseNet & 23.39\scalebox{0.7}{$\pm$2.17} & 0.765\scalebox{0.7}{$\pm$0.042} & 28.35\scalebox{0.7}{$\pm$2.30} & 0.845\scalebox{0.7}{$\pm$0.038} & 30.97\scalebox{0.7}{$\pm$2.33} & 0.902\scalebox{0.7}{$\pm$0.028}\\
    DuDoRNet & 18.46\scalebox{0.7}{$\pm$3.05} & 0.662\scalebox{0.7}{$\pm$0.093} & \textbf{37.88\scalebox{0.7}{$\pm$3.03}} & \textbf{0.985\scalebox{0.7}{$\pm$0.007}} & 30.53\scalebox{0.7}{$\pm$4.13} & 0.891\scalebox{0.7}{$\pm$0.071}\\
    Score SDE & 27.83\scalebox{0.7}{$\pm$2.73} & 0.849\scalebox{0.7}{$\pm$0.038} & 35.04\scalebox{0.7}{$\pm$2.11} & 0.943\scalebox{0.7}{$\pm$0.016} & 37.55\scalebox{0.7}{$\pm$2.08} & 0.960\scalebox{0.7}{$\pm$0.013}\\
    Langevin & 28.80\scalebox{0.7}{$\pm$3.21} & 0.873\scalebox{0.7}{$\pm$0.039} & 36.44\scalebox{0.7}{$\pm$2.28} & 0.952\scalebox{0.7}{$\pm$0.016} & 38.76\scalebox{0.7}{$\pm$2.32} & 0.966\scalebox{0.7}{$\pm$0.012}\\\hline \rowcolor{h}
    Ours & \textbf{29.42\scalebox{0.7}{$\pm$3.03}} & \textbf{0.880\scalebox{0.7}{$\pm$0.035}} & 37.63\scalebox{0.7}{$\pm$2.70} & 0.958\scalebox{0.7}{$\pm$0.015} & \textbf{39.91\scalebox{0.7}{$\pm$2.67}} & \textbf{0.965\scalebox{0.7}{$\pm$0.013}}\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    \end{adjustbox}
    }
\end{table}

\begin{table}
    \centering
    \definecolor{h}{gray}{0.9}
    \caption{Results for sparse-view CT reconstruction on LIDC and LDCT. FISTA-TV is a standard iterative reconstruction method that does not need training. cGAN, Neumann, and SIN-4c-PRN are supervised learning techniques trained with 23 projection angles.
    \label{tab:ct}}
    {\setlength{\extrarowheight}{1.5pt}
    \begin{adjustbox}{max width=0.8\textwidth}
    \begin{tabular}{c|c|cc|cc}
    \Xhline{3\arrayrulewidth}
    \multirow{2}{*}[-1pt]{Method} & \multirow{2}{*}[-1pt]{Projections} & \multicolumn{2}{c|}{LIDC $320\times 320$} & \multicolumn{2}{c}{LDCT $512\times 512$}\\\cline{3-6}
      &  & PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\
    \hline
    FBP & 23 & 10.18\scalebox{0.7}{$\pm$1.38} & 0.230\scalebox{0.7}{$\pm$0.072} & 10.11\scalebox{0.7}{$\pm$1.19} & 0.302\scalebox{0.7}{$\pm$0.078}\\
    FISTA-TV & 23 & 20.08\scalebox{0.7}{$\pm$4.89} & 0.799\scalebox{0.7}{$\pm$0.061} & 21.88\scalebox{0.7}{$\pm$4.42} & 0.850\scalebox{0.7}{$\pm$0.067}\\
    cGAN & 23 & 19.83\scalebox{0.7}{$\pm$3.07} & 0.479\scalebox{0.7}{$\pm$0.103} & 19.90\scalebox{0.7}{$\pm$2.52} & 0.545\scalebox{0.7}{$\pm$0.065}\\
    Neumann & 23 & 17.18\scalebox{0.7}{$\pm$3.79} & 0.454\scalebox{0.7}{$\pm$0.128} & 18.83\scalebox{0.7}{$\pm$3.29} & 0.525\scalebox{0.7}{$\pm$0.073}\\
    SIN-4c-PRN & 23 & 30.48\scalebox{0.7}{$\pm$3.99} & 0.895\scalebox{0.7}{$\pm$0.047} & 34.82\scalebox{0.7}{$\pm$3.55} & 0.877\scalebox{0.7}{$\pm$0.116}\\
    \hline \rowcolor{h}
    & 10 & 29.52\scalebox{0.7}{$\pm$2.63} & 0.823\scalebox{0.7}{$\pm$0.061} & 28.96\scalebox{0.7}{$\pm$4.41} & 0.849\scalebox{0.7}{$\pm$0.086} \\ \rowcolor{h}
     & 20 & 34.40\scalebox{0.7}{$\pm$2.66} & 0.895\scalebox{0.7}{$\pm$0.048} & 36.80\scalebox{0.7}{$\pm$4.50} & 0.936\scalebox{0.7}{$\pm$0.058}\\ \rowcolor{h}
     \multirow{-3}{*}{Ours} & 23 & \textbf{35.24\scalebox{0.7}{$\pm$2.71}} & \textbf{0.905\scalebox{0.7}{$\pm$0.046}} & \textbf{37.41\scalebox{0.7}{$\pm$4.62}} & \textbf{0.941\scalebox{0.7}{$\pm$0.057}}\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    \end{adjustbox}
    }
    \vspace{-1em}
\end{table}


\textbf{Supervised learning baselines}~
For sparse-view CT on both LIDC and LDCT, we include cGAN~\citep{ghani2018cgan}, Neumann~\citep{gilton2019neumann}, and SIN-4c-PRN~\citep{wei2020twostep} as supervised learning baselines. We follow the settings in \citet{wei2020twostep} and train all methods with 23 projection angles. For MAR, we use cGANMAR~\citep{wang2018conditional} and SNMAR~\citep{yu2020deep} as the baselines.
For undersampled MRI on BraTS, we compare against Cascade DenseNet~\citep{NEURIPS2019cascadenet} and DuDoRNet~\citep{zhou2020dudornet}, which are both trained with a $8\times$ acceleration factor by measuring only $1/8$ of the full k-space.

\textbf{Unsupervised learning baselines}~
For unsupervised techniques, so far only score-based generative models have witnessed success on clinic data. We compare with several existing methods that apply score-based generative models to inverse problem solving. Specifically, we consider the ``Langevin'' approach proposed in \citet{jalal2021robust}, and the ``Score SDE'' method in \citet{song2021scorebased}, where the former is limited to annealed Langevin dynamics (ALD) sampling, and the latter was based on a crude approximation to the conditional score function $\nabla_{\rvx_t} \log p_t(\rvx_t \mid \rvy)$ in \cref{eq:cond_reverse_sde}, and was proposed as a theoretical possibility in Appendix I.4 of \citet{song2021scorebased} without experiments. %
We only focus on undersampled MRI for these baselines, since it is the only medical imaging problem ever tackled with score-based generative models before our work. All methods share the same score models and only differ in terms of inference. We make sure all sampling algorithms have comparable number of iteration steps ($N$ in \cref{eq:iter,eq:iter2}).

\begin{wraptable}[8]{r}{0.35\textwidth}
    \vspace{-1em}
    \centering
    \definecolor{h}{gray}{0.9}
    \caption{MAR results on LIDC.\label{tab:mar}}
    {\setlength{\extrarowheight}{1.5pt}
    \begin{adjustbox}{max width=0.35\textwidth}
    \begin{tabular}{c|cc}
    \Xhline{3\arrayrulewidth}
    Method & PSNR$\uparrow$ & SSIM$\uparrow$ \\
    \hline
    LI & 26.30\scalebox{0.7}{$\pm$2.62} & 0.910\scalebox{0.7}{$\pm$0.028}\\
    cGANMAR & 27.27\scalebox{0.7}{$\pm$1.96} & 0.927\scalebox{0.7}{$\pm$0.060}\\
    SNMAR & 27.28\scalebox{0.7}{$\pm$1.43} & 0.937\scalebox{0.7}{$\pm$0.048}\\
    \hline \rowcolor{h}
    Ours & \textbf{32.16\scalebox{0.7}{$\pm$2.32}} & \textbf{0.939\scalebox{0.7}{$\pm$0.022}}\\
    \Xhline{3\arrayrulewidth}
    \end{tabular}
    \end{adjustbox}
    }
\end{wraptable}
\textbf{Competing with supervised learning approaches}~
Thanks to the outstanding sample quality of score-based generative models, we can achieve comparable or better performance than best-in-class supervised learning methods even for the same measurement process used in their training. As shown in \cref{tab:ct}, we outperform the top supervised learning technique SIN-4c-PRN on sparse-view CT reconstruction by a significant margin, on both the LIDC and LDCT datasets. Our results with 20 measurements are even better than supervised learning counterparts with 23 measurements. In \cref{fig:ct_demo}, we provide a visual comparison of the reconstruction quality for various methods, where it is clear to see that our method can recover more details faithfully. From results in \cref{tab:mar}, we also outperform the top supervised learning method SNMAR on metal artifact removal. As shown in \cref{fig:mar_demo}, our method generates images with less artifacts and preserves the structure better. For undersampled MRI reconstruction results given in \cref{tab:mar,tab:mri}, our method is ranked the 2nd for the case of $8\times$ acceleration, with comparable performance to the top supervised method DuDoRNet.


\textbf{Generalizing to different number of measurements}~
Since our approach is fully unsupervised, we can naturally apply the same score model to different measurement processes. We first consider changing the number of measurements at the test time, \eg, using different number of projection angles (\resp different acceleration factors) for sparse-view CT (\resp undersampled MRI) reconstruction. As shown in \cref{tab:mri} and \cref{fig:curves}~\figleft, we achieve the best performance on undersampled MRI for both $24\times$ and $4\times$ acceleration factors, whereas DuDoRNet fails to generalize when the acceleration factor changes. The other supervised learning approach Cascade DenseNet demonstrates limited adaptability by building a model architecture inspired by the physical measurement process of MRI, but fails to yield top-level performance. For sparse-view CT reconstruction, all supervised learning methods struggle to generalize to different projection angles, as shown in \cref{fig:curves}~\figcenter.


\textbf{Generalizing to different measurement processes in CT}~
We can perform both sparse-view CT reconstruction and metal artifact removal (MAR) with a single score model trained on CT images. These two tasks are inverse problems in CT imaging with different measurement processes $\mA$, but they share the same $\mT$ in the decomposition of \cref{prop:mask}. We provide a visualization of the measurement process corresponding to MAR in \cref{fig:medical_mar}.
As shown in \cref{tab:mar}, we can outperform supervised learning techniques specifically designed and trained for MAR, while using the same score model used in sparse-view CT reconstruction on LIDC.

\textbf{Comparing against existing score-based methods}~
We compare our method against Langevin~\citep{jalal2021robust} and Score SDE~\citep{song2021scorebased} for undersampled MRI reconstruction on BraTS. Two variants of our approach are considered, which respectively use annealed Langevin dynamics (ALD) and the Predictor-Corrector (PC) sampler for score-based generative models as the backend. We denote the former by ``ALD + Ours'', and the latter by ``PC + Ours'' (our default method for all other experiments). Recall that Langevin uses ALD as the sampler, same as ``ALD + Ours''. All results are provided in \cref{fig:curves}~\figright. We observe that ``ALD + Ours'' uniformly outperform Langevin and Score SDE across all numbers of measurements in the experiment. Moreover, ``PC + Ours'' can further improve ``ALD + Ours'', demonstrating the power of switching to more advanced sampling methods of score-based generative models in our proposed approach.














\begin{figure}
    \centering
    \includegraphics[width=0.33\linewidth]{figures/mri_psnr.png}%
    \includegraphics[width=0.33\linewidth]{figures/lidc_psnr.png}%
    \includegraphics[width=0.33\linewidth]{figures/ablation_psnr.png}
    \caption{Performance vs. numbers of measurements. Shaded areas represent standard deviation. \figleft~MRI on BraTS. \figcenter~CT on LIDC. \figright~Comparing score-based generative models for undersampled MRI reconstruction on BraTS. \label{fig:curves}}
\end{figure}

==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/intro.tex <==
\section{Introduction}
Computed Tomography (CT) and Magnetic Resonance Imaging (MRI) are commonly used imaging tools for medical diagnosis. Reconstructing CT and MRI images from raw measurements (sinograms for CT and k-spaces for MRI) are well-known inverse problems. Specifically, measurements in CT are given by X-ray projections of an object from various directions, and measurements in MRI are obtained by inspecting the Fourier spectrum of an object with magnetic fields. However, since obtaining the full sinogram for CT causes excessive ionizing radiation for patients, and measuring the full k-space of MRI is very time-consuming, it has become important to reduce the number of measurements in CT and MRI. In many cases, only partial measurements, such as sparse-view sinograms and downsampled k-spaces, are available. Due to this loss of information, the inverse problems in CT and MRI are often ill-posed, making image reconstruction especially challenging. 



With the rise of machine learning, many methods~\citep{zhu2018automap, mardani2017deep,shen2019patrecon, wurfl2018deepct, ghani2018cgan, wei2020twostep} have been proposed for medical image reconstruction using a small number of measurements. Most of these methods are supervised learning techniques. They learn to directly map partial measurements to medical images, by training on a large dataset comprising pairs of CT/MRI images and measurements. These measurements need to be synthesized from medical images with a fixed physical model of the measurement process. However, when the measurement process changes, such as using a different number of CT projections or different downsampling ratio of MRI k-spaces, we have to re-collect the paired dataset with the new measurement process and re-train the model. This prevents models from generalizing effectively to new measurement processes, leading to counter-intuitive instabilities such as more measurements causing worse performance~\citep{antun2020instabilities}.


In this work, we sidestep this difficulty completely by proposing unsupervised methods that do not require a paired dataset for training, and therefore are not restricted to a fixed measurement process. Our main idea is to learn the prior distribution of medical images with a generative model in order to infer the lost information due to partial measurements. Specifically, we propose to train a score-based generative model~\citep{song2019generative,song2020improved,song2021scorebased} on medical images as the data prior, due to its strong performance in image generation~\citep{ho2020denoising,dhariwal2021diffusion}. Given a trained score-based generative model, we provide a family of sampling algorithms to create image samples that are consistent with the observed measurements and the estimated data prior, leveraging the physical measurement process. Once our model is trained, it can be used to solve any inverse problem within the same image domain, as long as the mapping from images to measurements is linear, which holds for a large number of medical imaging applications.


We evaluate the performance of our method on several tasks in CT and MRI. Empirically, we observe comparable or better performance compared to supervised learning counterparts, even when evaluated with the same measurement process in their training. In addition, we are able to uniformly surpass all baselines when changing the number of measurements, \eg, using a different number of projections in sparse-view CT or changing the k-space downsampling ratio in undersampled MRI. Moreover, we show that by plugging in a different measurement process, we can use a single model to perform both sparse-view CT reconstruction and metal artifact removal for CT imaging with metallic implants. To the best of our knowledge, this is the first time that generative models are reported successful on clinical CT data. Collectively, these empirical results indicate that our method is a competitive alternative to supervised techniques in medical image reconstruction and artifact removal, and has the potential to be a universal tool for solving many inverse problems within the same image domain.














==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/libtheorems.tex <==
\usepackage{etoolbox}

\makeatletter

\newcommand{\define}[4][ignore]{%
  \ifstrequal{#1}{ignore}{}{
  \@namedef{thmtitle@#2}{#1}}%
  \@namedef{thm@#2}{#4}%
  \@namedef{thmtypen@#2}{lemma}%
  \newtheorem{thmtype@#2}[theorem]{#3}%
  \newtheorem*{thmtypealt@#2}{#3~\ref{#2}}%
}

\newcommand{\state}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
  \begin{thmtype@#1}
    }{
  \begin{thmtype@#1}[\@nameuse{thmtitle@#1}]
  }
    \label{#1}
    \@nameuse{thm@#1}
  \end{thmtype@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

\newcommand{\restate}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
    \begin{thmtypealt@#1}
    }{
  \begin{thmtypealt@#1}[\@nameuse{thmtitle@#1}]
  }
    \@nameuse{thm@#1}
  \end{thmtypealt@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

\newcommand{\thmlabel}[1]{
  \@ifundefined{thmdone@\@nameuse{curthm}}{\label{#1}
    }{\tag*{\eqref{#1}}}
}
\makeatother


==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/method.tex <==
\section{Solving inverse problems with score-based generative models}\label{sec:method}
\setlength{\fboxsep}{1pt}
\newcommand{\colorline}[1]{
\hspace{-0.03\linewidth}\colorbox{xkcdWine!30}{\makebox[0.99\linewidth][l]{#1}}
 }
\algnewcommand{\LineComment}[1]{\Statex \(\triangleright\) #1}
\begin{figure}
\begin{minipage}{.49\textwidth}
    \vspace{-0.7cm}
    \begin{algorithm}[H]
            \small
           \caption{Unconditional sampling}
           \label{alg:sampling}
            \begin{algorithmic}[1]
                \Require $N$
               \State $\hat{\rvx}_1 \sim \pi(\rvx), \Delta t \gets \frac{1}{N}$
               \For{$i=N-1$ {\bfseries to} $0$}
                 \State{$t \gets \frac{i+1}{N}$}
                 \item[]
                 \item[]
                 \item[]
                 \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t} - f(t) \hat{\rvx}_t \Delta t$}
                 \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t-\Delta t} + g(t)^2 \vs_{\vtheta^*}(\hat{\rvx}_{t}, t) \Delta t $}
                 \State{$\rvz \sim \mcal{N}(\bm{0}, \mI)$}
                 \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t-\Delta t} + g(t)\sqrt{\Delta t}~\rvz$}
               \EndFor
               \State {\bfseries return} $\hat{\rvx}_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\begin{minipage}{.49\textwidth}
    \vspace{-0.7cm}
    \begin{algorithm}[H]
            \small
           \caption{Inverse problem solving}
           \label{alg:inverse_problem}
            \begin{algorithmic}[1]
                \Require $N$, $\rvy$, $\lambda$
               \State $\hat{\rvx}_1 \sim \pi(\rvx), \Delta t \gets \frac{1}{N}$
               \For{$i=N-1$ {\bfseries to} $0$}
                 \State{$t \gets \frac{i+1}{N}$}
                 \State{\color{xkcdOrange}$\hat{\rvy}_{t} \sim p_{0t}(\rvy_t \mid \rvy)$}%
                 \State{\color{xkcdOrange}$
                    \hat{\rvx}_{t} \gets \mT^{-1}[\lambda \bm{\Lambda} \mcal{P}^{-1}(\bm{\Lambda})\hat{\rvy}_t + (1 - \lambda) \bm{\Lambda} \mT \hat{\rvx}_t + (\mI - \bm{\Lambda}) \mT \hat{\rvx}_t]$
                    }%
                \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t} - f(t) \hat{\rvx}_t \Delta t$}
                 \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t-\Delta t} + g(t)^2 \vs_{\vtheta^*}(\hat{\rvx}_{t}, t) \Delta t $}
                 \State{$\rvz \sim \mcal{N}(\bm{0}, \mI)$}
                 \State{$\hat{\rvx}_{t-\Delta t} \gets \hat{\rvx}_{t-\Delta t} + g(t)\sqrt{\Delta t}~\rvz$}%
               \EndFor
               \State {\bfseries return} $\hat{\rvx}_0$
            \end{algorithmic}
    \end{algorithm}
\end{minipage}
\vspace{-0.5em}
\end{figure}


With score-based generative modeling, we can train a score model $\vs_{\vtheta^*}(\rvx, t)$ to generate unconditional samples from the the prior distribution of medical images $p(\rvx)$. To solve inverse problems however, we will need to sample from the posterior $p(\rvx \mid \rvy)$. This can be accomplished by conditioning the original stochastic process $\{\rvx_t\}_{t\in[0,1]}$ on an observation $\rvy$, yielding a \emph{conditional} stochastic process $\{\rvx_t \mid \rvy\}_{t\in[0,1]}$. We denote the marginal distribution at $t$ as $p_t(\rvx_t \mid \rvy)$, and our goal is to sample from $p_0(\rvx_0 \mid \rvy)$, the same distribution as $p(\rvx \mid \rvy)$ by definition.
Much like generating unconditional samples by solving the reverse-time SDE in \cref{eq:reverse_sde}, we can reverse the conditional stochastic process $\{\rvx_t \mid \rvy\}_{t\in[0,1]}$ to sample from the posterior distribution $p_0(\rvx_0 \mid \rvy)$ by solving the following \emph{conditional} reverse-time SDE~\citep{song2021scorebased}:
\begin{align}
    \ud \rvx_t = \left[ f(t)\rvx_t - g(t)^{2} \nabla_{\rvx_t} \log p_{t}(\rvx_t \mid \rvy) \right] \ud t + g(t) \ud \bar{\rvw}_t,\qquad t\in[0,1]. \label{eq:cond_reverse_sde}
\end{align}
The conditional score function $\nabla_{\rvx_t} \log p_{t}(\rvx_t \mid \rvy)$ is a critical part of \cref{eq:cond_reverse_sde}, yet it is non-trivial to compute. One solution is to estimate the score function by training a new score model $\vs_{\vtheta^*}(\rvx_t, \rvy, t)$ that explicitly depends on $\rvy$~\citep{song2021scorebased,dhariwal2021diffusion}, such that $\vs_{\vtheta^*}(\rvx_t, \rvy, t) \approx \nabla_{\rvx_t} \log p_t(\rvx_t \mid \rvy)$. However, this requires paired data $\{(\rvx_i, \rvy_i)\}_{i=1}^N$ for training and has the same drawbacks as supervised learning techniques. We do not consider this approach in this work.

An unsupervised alternative is to approximate the conditional score function with an unconditionally-trained score model $\vs_{\vtheta^*}(\rvx_t, t) \approx \nabla_{\rvx_t} \log p_t(\rvx_t)$ and the measurement distribution $p(\rvy \mid \rvx)$. Many existing works \citep{song2021scorebased,kawar2021snips,kadkhodaie2020solving,jalal2021robust} have implemented this idea in different ways. %
However, the methods in \citet{kawar2021snips} and \citet{kadkhodaie2020solving} both require computing the singular value decomposition (SVD) of $\mA \in \mbb{R}^{m\times n}$, which can be difficult for many measurement processes in medical imaging. The method proposed in \citet{jalal2021robust} is only designed for a specific sampling method called annealed Langevin dynamics~\citep[ALD,][]{song2019generative}, which proves to be inferior to more advanced sampling algorithms such as Predictor-Corrector methods~\citep{song2021scorebased}. %

In what follows, we propose a new conditional sampling approach for inverse problem solving with score-based generative models. Our method is computationally efficient for medical image reconstruction, and is applicable to a large family of iterative sampling methods for score-based generative models. %
At a high level, we first train an unconditional score model $\vs_{\vtheta^*}(\rvx, t)$ on medical images without assuming any measurement process. Given an observation $\rvy$ at test time, we form a stochastic process $\{\rvy_t\}_{t\in[0,1]}$ by adding appropriate noise to $\rvy$. We then discretize the reverse-time SDE in \cref{eq:reverse_sde_model} with existing unconditional samplers for $\vs_{\vtheta^*}(\rvx, t)$, while incorporating the conditional information from $\rvy$ with a proximal optimization step to generate intermediate samples that are consistent with $\{\rvy_t\}_{t\in[0,1]}$.


\subsection{A convenient form of the linear measurement process}\label{sec:method:formulation}
Many different measurement processes in medical imaging share same components of computation. For example, sparse-view CT reconstruction and metal artifact removal for CT both involve computing the same Radon transform. Similarly, MRI measurement processes require computing the same spatial Fourier transform regardless of different downsampling ratios. To rigorously characterize this structure of measurement processes, we propose a special formulation of $\mA$ that is efficient to obtain in medical imaging applications. Without loss of generality, we assume that the linear operator $\mA$ has full rank, \ie, $\operatorname{rank}(\mA) = \min(n, m) = m$. The result below gives the alternative formulation of $\mA$:
\begin{restatable}{proposition}{prop}\label{prop:mask}
If $\operatorname{rank}(\mA) = m$, then there exist an invertible matrix $\mT \in \mbb{R}^{n\times n}$, and a diagonal matrix $\bm{\Lambda} \in \{0, 1\}^{n\times n}$ with $\operatorname{tr}(\bm{\Lambda}) = m$, such that $\mA = \mcal{P}(\bm{\Lambda}) \mT$. Here $\mcal{P}(\bm{\Lambda}) \in \{0, 1\}^{m\times n}$ is an operator that, when multiplied with any vector $\va \in \mbb{R}^n$, reduces its dimensionality to $m$ by removing each $i$-th element of $\va$ for $i=1,2,\cdots,n$ if $\bm{\Lambda}_{ii} = 0$.
\end{restatable}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/ct_def_new.png}\hfill
    \includegraphics[width=0.49\textwidth]{figures/mri_def_new.png}
    \caption{Linear measurement processes for sparse-view CT (\emph{left}) and undersampled MRI (\emph{right}). \label{fig:medical_inverse_probs}}
\end{figure}

We illustrate this decomposition for CT/MRI in \cref{fig:medical_inverse_probs}. Many measurement processes in medical imaging share the same $\mT$, even if they correspond to different $\mA$. For example, $\mT$ corresponds to the Radon transform and Fourier transform in sparse-view CT and undersampled MRI respectively, regardless of the number of measurements, \ie, CT projections and k-space downsampling ratios. For both sparse-view CT reconstruction and metal artifact removal for CT images, the operator $\mT$ is the Radon transform (see \cref{fig:medical_mar}). Intuitively, $\operatorname{diag}(\bm{\Lambda})$ can be viewed as a subsampling mask on the sinogram/k-space, and $\mcal{P}(\bm{\Lambda})$ subsamples the sinogram/k-space into an observation $\rvy$ with a smaller size according to this subsampling mask. In addition, we note that $\mT^{-1}$ can be efficiently implemented with the inverse Radon transform or the inverse Fourier transform in CT/MRI applications.


\subsection{Incorporating a given observation into an unconditional sampling process}
In what follows, we show that the decomposition in \cref{prop:mask} provides an efficient way to generate approximate samples from the conditional stochastic process $\{\rvx_t \mid \rvy\}_{t\in[0,1]}$ with an \emph{unconditional} score model $\vs_{\vtheta^*}(\rvx, t)$. The basic idea is to ``hijack'' the unconditional sampling process of score-based generative models to incorporate an observed measurement $\rvy$.


As we have already discussed, it is difficult to directly solve $\{\rvx_t \mid \rvy\}_{t\in[0,1]}$ for sample generation. To bypass this difficulty, we first consider a related stochastic process that is much easier to sample from. Recall that $p_{0t}(\rvx_t \mid \rvx_0) = \mcal{N}(\rvx_t \mid \alpha(t) \rvx_0, \beta^2(t)\mI)$ where $\alpha(t)$ and $\beta(t)$ can be derived from $f(t)$ and $g(t)$~\citep{song2021scorebased}. Given the unconditional stochastic process $\{\rvx_t \}_{t\in[0,1]}$, we define $\{\rvy_t\}_{t\in[0,1]}$, where $\rvy_t = \mA \rvx_t + \alpha(t) \bm{\epsilon}$. Unlike $\{\rvx_t \mid \rvy\}_{t\in[0,1]}$, the conditional stochastic process $\{\rvy_t \mid \rvy \}_{t\in[0,1]}$ is fully tractable. First, we have $\rvy_0 = \mA \rvx_0 + \alpha(0) \bm{\epsilon} = \mA \rvx_0 + \bm{\epsilon} = \rvy$. Since $p_{0t}(\rvx_t \mid \rvx_0) = \mcal{N}(\rvx_t \mid \alpha(t) \rvx_0, \beta^2(t)\mI)$, we have $\rvx_t=\alpha(t) \rvx_0 + \beta(t) \rvz$, where $\rvz \in \mbb{R}^n \sim \mcal{N}(\bm{0}, \bm{I})$. By definition, $\rvy_t=\mA \rvx_t + \alpha(t) \bm{\epsilon}$, so we have $\rvy_t = \mA (\alpha(t) \rvx_0 + \beta(t) \rvz) + \alpha(t) \bm{\epsilon} = \alpha(t) (\rvy - \bm{\epsilon}) + \beta(t) \mA \rvz + \alpha(t) \bm{\epsilon} = \alpha(t) \rvy + \beta(t)\mA \rvz$. %
Therefore, we can easily generate a sample $\hat{\rvy}_t \sim p_t(\rvy_t \mid \rvy)$ by first drawing $\rvz \sim \mcal{N}(\bm{0}, \bm{I})$ and then computing $\hat{\rvy}_t = \alpha(t) \rvy + \beta(t) \mA \rvz$.


The key of our approach is to modify any existing iterative sampling algorithm designed for the unconditional stochastic process $\{\rvx_t\}_{t\in[0,1]}$ so that the samples are consistent with $\{\rvy_t \mid \rvy\}_{t\in[0,1]}$. In general, an iterative sampling process of score-based generative models selects a sequence of time steps $\{0 = t_0 < t_1 < \cdots < t_N = 1\}$ and iterates according to
\begin{align}
    \hat{\rvx}_{t_{i-1}} = \vh(\hat{\rvx}_{t_i}, \rvz_i, \vs_{\vtheta^*}(\hat{\rvx}_{t_i}, t_i)), \quad i=N, N-1, \cdots, 1,\label{eq:iter}
\end{align}
where $\hat{\rvx}_{t_N} \sim \pi(\rvx)$, $\rvz_i \sim \mcal{N}(\bm{0}, \bm{I})$, and $\vtheta^*$ denotes the parameters in an unconditional score model $\vs_{\vtheta^*}(\rvx, t)$. Here the iteration function $\vh$ takes a noisy sample $\hat{\rvx}_{t_i}$ and reduces the noise therein to generate $\hat{\rvx}_{t_{i-1}}$, using the unconditional score model $\vs_{\vtheta^*}(\rvx, t)$. For example, for the Euler-Maruyama sampler detailed in \cref{alg:sampling}, this iteration function is given by
\begin{align*}
    \vh(\hat{\rvx}_{t_i}, \rvz_i, \vs_{\vtheta^*}(\hat{\rvx}_{t_i}, t_i)) = \hat{\rvx}_{t_i} - f(t_i)\hat{\rvx}_{t_i}/N + g(t_i)^2 \vs_{\vtheta^*}(\hat{\rvx}_{t_i}, t_i)/N + g(t_i)\rvz_i/\sqrt{N}.
\end{align*}
Samples obtained by this procedure $\{\hat{\rvx}_{t_i}\}_{i=0}^N$ constitute an approximation of $\{\rvx_t\}_{t\in[0,1]}$, where the last sample $\hat{\rvx}_{t_0}$ can be viewed as an approximate sample from $p_0(\rvx)$. %
Most existing sampling methods for score-based generative models are instances of this iterative sampling paradigm, including \cref{alg:sampling}, ALD~\citep{song2019generative}, probability flow ODEs~\citep{song2021scorebased} and Predictor-Corrector samplers~\citep{song2021scorebased}.


To enforce the constraint implied by $\{\rvy_t \mid \rvy\}_{t\in[0,1]}$, we prepend an additional step to the iteration rule in \cref{eq:iter}, leading to
\begin{align}
    \hat{\rvx}_{t_i}' &= \vk(\hat{\rvx}_{t_{i}}, \hat{\rvy}_{t_i}, \lambda)\\
    \hat{\rvx}_{t_{i-1}} &= \vh(\hat{\rvx}_{t_i}', \rvz_i, \vs_{\vtheta^*}(\hat{\rvx}_{t_i}, t_i)), \quad i=N,N-1,\cdots, 1,
    \label{eq:iter2}
\end{align}
where $\hat{\rvx}_{t_N} \sim \pi(\rvx)$, $\hat{\rvy}_{t_i} \sim p_{t_i}(\rvy_{t_i} \mid \rvy)$, and $0\leq \lambda \leq 1$ is a hyper-parameter. We provide an illustration of this process in \cref{fig:projection}. The iteration function $\vk(\cdot, \hat{\rvy}_{t_i}, \lambda): \mbb{R}^n \to \mbb{R}^n$ promotes data consistency by %
solving a proximal optimization step~\citep{nesterov2003introductory,boyd2004convex,hammernik2021systematic} that simultaneously minimizes the distance between $\hat{\rvx}_{t_i}'$ and $\hat{\rvx}_{t_i}$, and the distance between $\hat{\rvx}_{t_i}'$ and the hyperplane $\{\vx \in \mbb{R}^n \mid \mA \vx = \hat{\rvy}_{t_{i}}\}$, with a hyperparameter $0 \leq \lambda \leq 1$ balancing between the two:
\begin{align}
    \hat{\rvx}_{t_i}' = \argmin_{\vz \in \mbb{R}^n} \{ (1- \lambda) \norm{\vz - \hat{\rvx}_{t_i}}_\mT^2 + \min_{\vu \in \mbb{R}^n}\lambda \norm{\vz - \vu}_\mT^2\} \quad s.t.  \quad  \mA \vu = \hat{\rvy}_{t_i}. \label{eq:optimize}
\end{align}
Recall that $\mA = \mcal{P}(\bm{\Lambda})\mT$ according to \cref{prop:mask}. In the equation above we choose the norm $\norm{\va}_\mT^2 \coloneqq \norm{\mT \va}_2^2$ to simplify our theoretical analysis. The decomposition in \cref{prop:mask} allows us to derive a closed-form solution to the optimization problem in \cref{eq:optimize}, as given below:%
\begin{restatable}{theorem}{thm}\label{theorem}
The solution of \cref{eq:optimize} can be given by
\begin{align}
    \hat{\rvx}_{t_i}' = \mT^{-1}[\lambda \bm{\Lambda} \mcal{P}^{-1}(\bm{\Lambda})\hat{\rvy}_{t_i} + (1 - \lambda) \bm{\Lambda} \mT \hat{\rvx}_{t_i} + (\mI - \bm{\Lambda}) \mT \hat{\rvx}_{t_i}],
\end{align}
where $\mcal{P}^{-1}(\bm{\Lambda}): \mbb{R}^m \to \mbb{R}^n$ denotes any right inverse of $\mcal{P}(\bm{\Lambda})$. %
\end{restatable}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/method_schematic.jpg}
    \caption{\figleft{} An overview of our method for solving inverse problems with score-based generative models. \figright{} An illustration about how to combine $\hat{\rvx}_{t_i}$ and $\rvy$ to form $\hat{\rvx}_{t_i}'$.%
    }
    \label{fig:projection}
\end{figure}

See \cref{fig:projection} for an illustration of the function $\hat{\rvx}_{t_i}' = \vk(\hat{\rvx}_{t_i}, \hat{\rvy}_{t_i}, \lambda)$. The right inverse $\mcal{P}^{-1}(\bm{\Lambda})$ increases the dimensionality of a vector $\va\in\mbb{R}^m$ to $n$ by putting its entries on every index $i$ of an $n$-dimensional vector where $\bm{\Lambda}_{ii} = 1$. Recall that in sparse-view CT or undersampled MRI, $\operatorname{diag}(\bm{\Lambda})$ represents a subsampling mask, and $\mcal{P}(\bm{\Lambda})$ subsamples the full sinogram/k-space to generate the observation $\rvy$. In this case, $\mcal{P}^{-1}(\bm{\Lambda})$ pads the observation $\rvy$ so that it has the same size as the full sinogram/k-space. 

When $\lambda = 0$, $\hat{\rvx}_{t_i}' = \vk(\hat{\rvx}_{t_i}, \hat{\rvy}_{t_i}, 0) = \hat{\rvx}_{t_i}$ completely ignores the constraint $\mA \hat{\rvx}_{t_i}' = \hat{\rvy}_{t_i}$, in which case our sampling method in \cref{eq:iter2} performs unconditional generation. On the other hand, when $\lambda=1$, $\hat{\rvx}_{t_i}' = \vk(\hat{\rvx}_{t_i}, \hat{\rvy}_{t_i}, 1)$ satisfies $\mA \hat{\rvx}_{t_i}' = \hat{\rvy}_{t_i}$ exactly. When the measurement is noisy, we choose $0 < \lambda < 1$ to allow slackness in the constraint $\mA \hat{\rvx}_{t_i}' = \hat{\rvy}_{t_i}$. %
The value of $\lambda$ is important for balancing between $\hat{\rvx}_{t_i}' \approx \hat{\rvx}_{t_i}$ and $\mA \hat{\rvx}_{t_i}' \approx \hat{\rvy}_{t_i}$. In practice, we use Bayesian optimization to tune this $\lambda$ automatically on a validation dataset. When the measurement process contains no noise, we replace $\hat{\rvx}_{t_0}$ with $\vk(\hat{\rvx}_{t_0}, \rvy, 1)$ at the last sampling step to guarantee $\mA \hat{\rvx}_{t_0} = \rvy$. 

In summary, our method given in \cref{eq:iter2} introduces minimal modifications to an existing iterative sampling method of score-based generative models. For example, we can convert the sampler in \cref{alg:sampling} to an inverse problem solver in \cref{alg:inverse_problem} by adding/modifying just three lines of pseudo-code. Unlike the concurrent work~\citet{jalal2021robust}, our method is not limited to annealed Langevin dynamics (ALD).  As demonstrated in our experiments, we outperform \citet{jalal2021robust} even with the same ALD sampler, and can widen the performance gap further by using more advanced approaches like the Predictor-Corrector sampler~\citep{song2021scorebased}. Unlike \citet{kadkhodaie2020solving,kawar2021snips}, we rely on the efficient alternative representation of $\mA$ given in \cref{sec:method:formulation}, and do not require expensive SVD computation. %





==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/related_work.tex <==
\section{Related Work}
The idea of solving inverse problems with generative models has been proposed in the Compressed Sensing with Generative Models (CSGM) framework~\citep{bora2017compressed}. However, the original CSGM method is centered around latent variable models such as Generative Adversarial Networks \citep[GANs,][]{goodfellow2014generative} and Variational Auto-Encoders \cite[VAEs,][]{kingma-AutoEncodingVariationalBayes-2014,rezende-StochasticBackpropagationApproximate-2014}. It is unclear how to apply CSGM to other families of generative models like Energy-Based Models \citep[EBMs,][]{song2021train} and score-based generative models.

SNIPS~\cite{kawar2021snips} (solving noisy inverse problem stochastically).

Solving linear inverse problems with unsupervised learning and denoising score matching~\citep{vincent2011connection} has also been explored in \citet{kadkhodaie2020solving}. In contrast with our approach, their method requires projecting an noisy sample onto the kernel space of a linear operator, which can be expensive to compute for high dimensional data. They did not consider applications in medical imaging either.

Concurrently, \citet{jalal2020robust} extends the NCSNv2 model~\citep{song2020improved}, a score-based generative model sampled by annealed Langevin dynamics~\citep{song2019generative}, to solve inverse problems in downsampled MRI reconstruction. Our method is applicable to more general sampling methods~\citep{song2021scorebased} for score-based generative models, such as numerical SDE solvers, Predictor-Corrector samplers, and probability flow ODE samplers. We also obtained uniformly better empirical performance in our experiments.



==> Solving Inverse Problems in Medical Imaging with Score-Based Generative Models_arXiv/results.tex <==
\section{Results}





==> libtheorems.tex <==
\usepackage{etoolbox}

\makeatletter

\newcommand{\define}[4][ignore]{%
  \ifstrequal{#1}{ignore}{}{
  \@namedef{thmtitle@#2}{#1}}%
  \@namedef{thm@#2}{#4}%
  \@namedef{thmtypen@#2}{lemma}%
  \newtheorem{thmtype@#2}[theorem]{#3}%
  \newtheorem*{thmtypealt@#2}{#3~\ref{#2}}%
}

\newcommand{\state}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
  \begin{thmtype@#1}
    }{
  \begin{thmtype@#1}[\@nameuse{thmtitle@#1}]
  }
    \label{#1}
    \@nameuse{thm@#1}
  \end{thmtype@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

\newcommand{\restate}[1]{%
  \@namedef{curthm}{#1}
  \@ifundefined{thmtitle@#1}{
    \begin{thmtypealt@#1}
    }{
  \begin{thmtypealt@#1}[\@nameuse{thmtitle@#1}]
  }
    \@nameuse{thm@#1}
  \end{thmtypealt@#1}
  \@ifundefined{thmdone@#1}{
  \@namedef{thmdone@#1}{stated}%
  }{}
}

\newcommand{\thmlabel}[1]{
  \@ifundefined{thmdone@\@nameuse{curthm}}{\label{#1}
    }{\tag*{\eqref{#1}}}
}
\makeatother


==> related_work.tex <==
\section{Related Work}
The idea of solving inverse problems with generative models has been proposed in the Compressed Sensing with Generative Models (CSGM) framework~\citep{bora2017compressed}. However, the original CSGM method is centered around latent variable models such as Generative Adversarial Networks \citep[GANs,][]{goodfellow2014generative} and Variational Auto-Encoders \cite[VAEs,][]{kingma-AutoEncodingVariationalBayes-2014,rezende-StochasticBackpropagationApproximate-2014}. It is unclear how to apply CSGM to other families of generative models like Energy-Based Models \citep[EBMs,][]{song2021train} and score-based generative models.

SNIPS~\cite{kawar2021snips} (solving noisy inverse problem stochastically).

Solving linear inverse problems with unsupervised learning and denoising score matching~\citep{vincent2011connection} has also been explored in \citet{kadkhodaie2020solving}. In contrast with our approach, their method requires projecting an noisy sample onto the kernel space of a linear operator, which can be expensive to compute for high dimensional data. They did not consider applications in medical imaging either.

Concurrently, \citet{jalal2020robust} extends the NCSNv2 model~\citep{song2020improved}, a score-based generative model sampled by annealed Langevin dynamics~\citep{song2019generative}, to solve inverse problems in downsampled MRI reconstruction. Our method is applicable to more general sampling methods~\citep{song2021scorebased} for score-based generative models, such as numerical SDE solvers, Predictor-Corrector samplers, and probability flow ODE samplers. We also obtained uniformly better empirical performance in our experiments.



==> results.tex <==
\section{Results}




